T-DominO: Exploring Multiple Criteria with Quality-Diversity and the Tournament Dominance Objective

Real-world design problems are a messy combination of constraints, objectives, and features. Exploring these problem spaces can be defined as a Multi-Criteria Exploration (MCX) problem, whose goals are to produce a set of diverse solutions with high performance across many objectives, while avoiding low performance across any objectives. Quality-Diversity algorithms produce the needed design variation, but typically consider only a single objective. We present a new ranking, T-DominO, specifically designed to handle multiple objectives in MCX problems. T-DominO ranks individuals relative to other solutions in the archive, favoring individuals with balanced performance over those which excel at a few objectives at the cost of the others. Keeping only a single balanced solution in each MAP-Elites bin maintains the visual accessibility of the archive -- a strong asset for design exploration. We illustrate our approach on a set of easily understood benchmarks, and showcase its potential in a many-objective real-world architecture case study.

==> tex/fig_03_cycling.tex <==
\begin{figure}[t]
  \centering
  \vspace{-0.2cm}
  \includegraphics[width=\figscale\textwidth,center]{img/03_cycling.png}
  \caption
  { 
  %\newline
    \textbf{Using historical solutions to prevent cycling in T-DominO.} T-DominO ranks individuals based on their dominance of each other solution in each objective. To prevent oscillation between non-dominated solutions the history of previous elites' objective values is used to compute T-DominO in each bin.
  }
  \label{fig:cycling}
\end{figure}

==> tex/fig_06_wfcOpt.tex <==
\begin{figure}[th!]
  \centering
  \vspace{-0.2cm}
  \includegraphics[width=\figscale\textwidth,center]{img/06_wfc_opt.png}
  \caption
  { 
  %\newline
    \textbf{A visual explanation.} You should be able to read the paper with just figures.
  }
  \label{fig:overview}
\end{figure}
